OpenCUA: Open Foundations for Computer-Use Agents

Vision-language models have demonstrated impressive capabilities as computer-use agents (CUAs) capable of automating diverse computer tasks. As their commercial potential grows, critical details of the most capable CUA systems remain closed. As these agents will increasingly mediate digital interactions and execute consequential decisions on our behalf, the research community needs access to open CUA frameworks to study their capabilities, limitations, and risks. To bridge this gap, we propose OpenCUA, a comprehensive open-source framework for scaling CUA data and foundation models. Our framework consists of: (1) an annotation infrastructure that seamlessly captures human computer-use demonstrations; (2) AgentNet, the first large-scale computer-use task dataset spanning 3 operating systems and 200+ applications and websites; (3) a scalable pipeline that transforms demonstrations into state-action pairs with reflective long Chain-of-Thought reasoning that sustain robust performance gains as data scales. Our end-to-end agent models demonstrate strong performance across CUA benchmarks. In particular, OpenCUA-72B achieves an average success rate of 45.0% on OSWorld-Verified, establishing a new state-of-the-art (SOTA) among open-source models. Further analysis confirms that our approach generalizes well across domains and benefits significantly from increased test-time computation. We release our annotation tool, datasets, code, and models to build open foundations for further CUA research.

==> tables/osworld_main.tex <==
\begin{table}[t]
\vspace{-20pt}
\caption{Online evaluation results on OSWorld~\citep{OSWorld} and
       WindowsAgentArena (WAA)~\citep{bonatti2024windowsagentarenaevaluating}. Reported OpenCUA scores are the mean of 4 independent runs.}
       % \tao{uitars1.5, no papers/details - footnote to explain why not included, reported results? - openai operator?}

\centering
  \small
  % tighter padding & row height
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.12}
  \begin{tabular}{llcccc}
    \toprule
    \textbf{Agent Model} &                &
      \multicolumn{2}{c}{\textbf{OSWorld}} &
      \multicolumn{2}{c}{\textbf{WAA}} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    & & 15 steps & 50 steps & 15 steps & 50 steps \\ \midrule
    % \multicolumn{6}{l}{\textbf{Agent Model}} \\ \midrule
      Qwen-2.5-VL-7B~\citep{bai2025qwen2.5vl}       & &  2.5 & --  & --  & --  \\
      Qwen-2.5-VL-32B~\citep{bai2025qwen2.5vl}       & &  5.9 & --  & --  & --  \\
      % Gemini-Pro-1.5~\citep{team2024gemini}          & &  5.4 & --  & --  & --  \\
      % CogAgent-9B-20241220~\citep{hong2024cogagent}  & &  8.1 & --  & --  & --  \\
      Qwen-2.5-VL-72B~\citep{bai2025qwen2.5vl}       & &  8.8 & --  & --  & --  \\
      Kimi-VL-A3B~\citep{team2025kimi}               & &  8.2 & --  & \underline{10.4}& --  \\
      Aguvis-72B~\citep{xu2024aguvis}                & & 10.3 & --  & --  & --  \\
      
      UI-TARS-7B-DPO~\citep{qin2025uitarspioneeringautomatedgui}
                                                     & & 18.7 & --  & --  & --  \\
      UI-TARS-72B-DPO~\citep{qin2025uitarspioneeringautomatedgui}
                                                     & & \underline{22.7} & 24.6  & --  & --  \\
      Claude 3.7 Sonnet~\citep{anthropic_claude_use_2024} & & 15.5 & 26.0& --  & --  \\
      OpenAI CUA~\citep{openai_operator_2025}     & & 19.7 & \underline{32.6}  & --  & --  \\
      \addlinespace
      % \textbf{OpenCUA-A3B}  & & 15.5 & 17.3 & 16.0 & 17.5 \\
      % \textbf{OpenCUA-7B}   & & 18.5& 20.1 & 16.1 & 21.1 \\
      % \textbf{OpenCUA-2.5-7B}  & & 21.8 & 25.3 & 22.5 & 27.1 \\
      % \textbf{OpenCUA-2.5-32B}   & & \textbf{24.4}& \textbf{27.7} & \textbf{23.8}& \textbf{28.0} \\
      \midrule
        \multicolumn{5}{l}{\textbf{Our Scaffolding}} \\
        \midrule
      OpenCUA-A3B  & &
          15.5$_{\pm0.84}$ & 17.3$_{\pm0.50}$ &
          16.0$_{\pm1.33}$ & 17.5$_{\pm0.74}$ \\
        
        OpenCUA-Qwen2-7B   & &
          18.5$_{\pm1.22}$ & 20.1$_{\pm2.12}$ &
          16.1$_{\pm2.02}$ & 21.1$_{\pm2.03}$ \\
        
        OpenCUA-7B & &
          21.8$_{\pm1.50}$ & 25.3$_{\pm0.50}$ &
          22.5$_{\pm0.80}$ & 27.1$_{\pm2.80}$ \\
        
        OpenCUA-32B & &
          \textbf{26.2}$_{\pm1.00}$ & \textbf{30.1}$_{\pm0.91}$ &
          \textbf{23.8}$_{\pm1.50}$ & \textbf{28.0}$_{\pm2.00}$ \\
    \bottomrule
  \end{tabular}
  \label{tab:online_osworld}
\vspace{-15pt}
\end{table}



==> tables/osworld_results.tex <==

\begin{table}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{Detailed performance of OpenCUA models on \osworld{} (mean of 4 runs unless noted).}
\label{tab:opencua_detailed}

\begin{tabular}{c l|c|cccccccccc|cc}
\toprule
\textbf{Model} & \textbf{#Step} & \textbf{Overall} &
\textbf{LibreCalc} & \textbf{Impress} & \textbf{Writer} & \textbf{Chrome} &
\textbf{VLC} & \textbf{TB} & \textbf{OS} & \textbf{GIMP} &
\textbf{VSCode} & \textbf{MultiApp} &
\makecell{\textbf{Succ.~Len}} &
\makecell{\textbf{Fail~Len}} \\
\midrule
% -------------------- 7B : 15 --------------------
& \textbf{15 Steps} & & & & & & & & & & & & & \\
& Run 1 & 21.05 & 3 & 14 & 6 & 13 & 3 & 3 & 9 & 10 & 9 & 6 & 6.96 & 12.84 \\
& Run 2 & 23.27 & 3 & 13 & 8 & 16 & 3 & 4 & 9 & 9 & 11 & 8 & 7.30 & 12.67 \\
& Run 3 & 20.78 & 5 & 11 & 6 & 14 & 3 & 4 & 7 & 9 & 10 & 6 & 6.85 & 12.53 \\
& Run 4 & 21.94 & 5 & 12 & 8 & 12 & 5 & 4 & 8 & 8 & 11 & 6 & 7.08 & 12.74 \\
& \textit{Avg} & 21.76 & 4.0 & 12.5 & 7.0 & 13.8 & 3.5 & 3.8 & 8.3 & 9.0 & 10.3 & 6.5 & 7.05 & 12.70 \\
\cmidrule(lr){2-15}
% -------------------- 7B : 30 --------------------
& \textbf{30 Steps} & & & & & & & & & & & & & \\
& Run 1 & 22.01 & 4 & 10 & 6 & 15 & 4 & 4 & 7 & 10 & 11 & 8 & 8.48 & 18.65 \\
& Run 2 & 24.10 & 7 & 13 & 7 & 15 & 3 & 5 & 9 & 8 & 12 & 8 & 9.20 & 18.43 \\
OpenCUA‑7B & Run 3 & 23.27 & 7 & 13 & 6 & 14 & 3 & 4 & 10 & 9 & 11 & 7 & 8.08 & 18.93 \\
& Run 4 & 22.44 & 5 & 11 & 7 & 15 & 4 & 3 & 10 & 7 & 12 & 7 & 8.01 & 18.06 \\
& \textit{Avg} & 22.96 & 5.8 & 11.8 & 6.5 & 14.8 & 3.5 & 4.0 & 9.0 & 8.5 & 11.5 & 7.5 & 8.44 & 18.52 \\
\cmidrule(lr){2-15}
% -------------------- 7B : 50 --------------------
& \textbf{50 Steps} & & & & & & & & & & & & & \\
& Run 1 & 24.93 & 7 & 13 & 9 & 15 & 3 & 3 & 10 & 9 & 12 & 9 & 9.11 & 23.23 \\
& Run 2 & 25.83 & 5 & 14 & 7 & 17 & 4 & 4 & 10 & 10 & 12 & 10 & 9.33 & 21.90 \\
& Run 3 & 25.21 & 8 & 13 & 9 & 16 & 5 & 3 & 8 & 9 & 12 & 8 & 9.37 & 23.22 \\
& Run 4 & 25.21 & 6 & 12 & 10 & 16 & 3 & 5 & 8 & 9 & 12 & 10 & 9.43 & 22.71 \\
& \textit{Avg} & 25.30 & 6.5 & 13.0 & 8.8 & 16.0 & 3.8 & 3.8 & 9.0 & 9.3 & 12.0 & 9.3 & 9.31 & 22.77 \\
\midrule
% ==================== 32B : 15 ====================
& \textbf{15 Steps} & & & & & & & & & & & & & \\
& Run 1 & 27.22 & 8 & 14 & 10 & 11 & 5 & 7 & 8 & 10 & 13 & 12 & 6.85 & 12.41 \\
& Run 2 & 25.07 & 4 & 14 & 9 & 15 & 3 & 7 & 9 & 9 & 11 & 9 & 6.63 & 12.42 \\
& Run 3 & 25.98 & 7 & 13 & 8 & 16 & 4 & 6 & 7 & 10 & 12 & 10 & 6.96 & 12.38 \\
& Run 4 & 26.46 & 5 & 15 & 9 & 16 & 4 & 6 & 7 & 10 & 13 & 10 & 6.69 & 12.34 \\
& \textit{Avg} & 26.18 & 6.0 & 14.0 & 9.0 & 14.5 & 4.0 & 6.5 & 7.8 & 9.8 & 12.3 & 10.3 & 6.78 & 12.39 \\
\cmidrule(lr){2-15}
% -------------------- 32B : 30 --------------------
& \textbf{30 Steps} & & & & & & & & & & & & & \\
& Run 1 & 29.89 & 6 & 17 & 11 & 21 & 5 & 7 & 8 & 9 & 12 & 11 & 7.52 & 18.41 \\
& Run 2 & 30.08 & 8 & 18 & 10 & 19 & 3 & 7 & 10 & 12 & 13 & 8 & 7.95 & 17.97 \\
OpenCUA‑32B & Run 3 & 29.53 & 8 & 15 & 9 & 19 & 4 & 7 & 10 & 9 & 12 & 13 & 8.35 & 18.41 \\
& Run 4 & 27.93 & 7 & 13 & 9 & 19 & 3 & 6 & 11 & 9 & 12 & 11 & 7.53 & 18.40 \\
& \textit{Avg} & 29.36 & 7.3 & 15.8 & 9.8 & 19.5 & 3.8 & 6.8 & 9.8 & 9.8 & 12.3 & 10.8 & 7.84 & 18.30 \\
\cmidrule(lr){2-15}
% -------------------- 32B : 50 --------------------
& \textbf{50 Steps} & & & & & & & & & & & & & \\
& Run 1 & 29.81 & 7 & 15 & 11 & 20 & 6 & 8 & 8 & 9 & 13 & 10 & 8.61 & 22.54 \\
& Run 2 & 29.17 & 8 & 16 & 9 & 19 & 4 & 7 & 7 & 11 & 12 & 12 & 8.57 & 21.61 \\
& Run 3 & 31.01 & 5 & 17 & 10 & 20 & 6 & 8 & 12 & 10 & 12 & 11 & 8.81 & 22.81 \\
& Run 4 & 30.56 & 8 & 14 & 10 & 18 & 4 & 7 & 11 & 12 & 13 & 13 & 8.80 & 22.62 \\
& \textit{Avg} & 30.14 & 7.0 & 15.5 & 10.0 & 19.3 & 5.0 & 7.5 & 9.5 & 10.5 & 12.5 & 11.5 & 8.70 & 22.40 \\
\midrule
% ==================== A3B : 15 ====================
& \textbf{15 Steps} & & & & & & & & & & & & & \\
& Run 1 & 15.32 & 3 & 8 & 2 & 14 & 2 & 2 & 2 & 7 & 10 & 5 & 7.38 & 12.20 \\
& Run 2 & 15.60 & 2 & 9 & 6 & 13 & 3 & 2 & 3 & 7 & 8 & 3 & 7.11 & 12.18 \\
& Run 3 & 14.68 & 2 & 7 & 5 & 13 & 3 & 1 & 2 & 8 & 8 & 4 & 6.68 & 12.27 \\
& Run 4 & 16.34 & 3 & 6 & 5 & 15 & 3 & 3 & 3 & 9 & 10 & 2 & 7.22 & 12.28 \\
& \textit{Avg} & 15.50 & 2.5 & 7.5 & 4.5 & 13.75 & 2.75 & 2.0 & 2.5 & 7.75 & 9.0 & 3.5 & 7.10 & 12.23 \\
\cmidrule(lr){2-15}
% -------------------- A3B : 30 --------------------
& \textbf{30 Steps} & & & & & & & & & & & & & \\
& Run 1 & 16.94 & 2 & 8 & 4 & 12 & 3 & 6 & 6 & 8 & 11 & 1 & 9.02 & 17.38 \\
& Run 2 & 17.50 & 2 & 7 & 3 & 16 & 3 & 2 & 8 & 6 & 11 & 5 & 8.17 & 17.55 \\
OpenCUA-A3B & Run 3 & 17.78 & 2 & 7 & 6 & 15 & 3 & 4 & 5 & 8 & 10 & 4 & 8.59 & 17.85 \\
& Run 4 & 15.79 & 2 & 8 & 6 & 12 & 3 & 2 & 3 & 7 & 10 & 4 & 7.89 & 17.63 \\
& \textit{Avg} & 17.00 & 2.0 & 7.5 & 4.75 & 13.75 & 3.0 & 3.5 & 5.5 & 7.25 & 10.5 & 3.5 & 8.42 & 17.60 \\
\cmidrule(lr){2-15}
% -------------------- A3B : 50 --------------------
& \textbf{50 Steps} & & & & & & & & & & & & & \\
& Run 1 & 17.32 & 3 & 7 & 5 & 15 & 5 & 2 & 4 & 7 & 8 & 6 & 9.10 & 19.48 \\
& Run 2 & 16.43 & 3 & 8 & 4 & 14 & 3 & 2 & 2 & 8 & 10 & 5 & 7.25 & 20.34 \\
& Run 3 & 17.83 & 4 & 9 & 5 & 13 & 3 & 3 & 5 & 8 & 10 & 4 & 7.44 & 21.27 \\
& Run 4 & 17.55 & 2 & 7 & 7 & 14 & 3 & 1 & 6 & 9 & 9 & 5 & 8.33 & 20.98 \\
& \textit{Avg} & 17.28 & 3.0 & 7.75 & 5.25 & 14.00 & 3.5 & 2.0 & 4.25 & 8.00 & 9.25 & 5.0 & 8.03 & 20.52 \\
\midrule
% ==================== Qwen2-7B : 15 ====================
& \textbf{15 Steps} & & & & & & & & & & & & & \\
& Run 1 & 16.67 & 3 & 9 & 8 & 7 & 3 & 5 & 6 & 8 & 11 & 0 & 7.27 & 12.61 \\
& Run 2 & 18.06 & 3 & 10 & 8 & 15 & 2 & 4 & 4 & 8 & 10 & 1 & 7.72 & 12.76 \\
& Run 3 & 16.16 & 4 & 8 & 8 & 10 & 2 & 4 & 4 & 8 & 9 & 1 & 7.28 & 12.60 \\
& Run 4 & 16.39 & 4 & 9 & 8 & 10 & 3 & 4 & 2 & 9 & 8 & 2 & 7.49 & 12.45 \\
& \textit{Avg} & 16.82 & 3.5 & 9.0 & 8.0 & 10.5 & 2.5 & 4.25 & 4.0 & 8.25 & 9.5 & 1.0 & 7.44 & 12.61 \\
\cmidrule(lr){2-15}
% -------------------- Qwen2-7B : 30 --------------------
& \textbf{30 Steps} & & & & & & & & & & & & & \\
& Run 1 & 17.50 & 3 & 7 & 9 & 12 & 4 & 6 & 4 & 7 & 9 & 2 & 7.75 & 18.40 \\
& Run 2 & 17.60 & 4 & 8 & 6 & 8 & 4 & 7 & 6 & 6 & 10 & 4 & 8.92 & 17.98 \\
OpenCUA-Qwen2-7B & Run 3 & 16.43 & 6 & 6 & 6 & 10 & 3 & 4 & 1 & 9 & 9 & 5 & 9.17 & 19.07 \\
& Run 4 & 18.61 & 3 & 8 & 8 & 11 & 5 & 4 & 5 & 9 & 9 & 5 & 9.09 & 18.12 \\
& \textit{Avg} & 17.54 & 4.0 & 7.25 & 7.25 & 10.25 & 4.0 & 5.25 & 4.0 & 7.75 & 9.25 & 4.0 & 8.73 & 18.39 \\
\cmidrule(lr){2-15}
% -------------------- Qwen2-7B : 50 --------------------
& \textbf{50 Steps} & & & & & & & & & & & & & \\
& Run 1 & 19.22 & 5 & 8 & 9 & 14 & 3 & 4 & 4 & 9 & 9 & 4 & 8.86 & 22.86 \\
& Run 2 & 20.56 & 3 & 9 & 8 & 14 & 3 & 7 & 8 & 7 & 11 & 4 & 9.27 & 22.16 \\
& Run 3 & 19.17 & 3 & 8 & 6 & 12 & 3 & 6 & 5 & 10 & 12 & 4 & 9.32 & 20.98 \\
& Run 4 & 20.06 & 3 & 14 & 10 & 13 & 5 & 5 & 3 & 7 & 8 & 4 & 9.68 & 22.73 \\
& \textit{Avg} & 19.75 & 3.5 & 9.75 & 8.25 & 13.25 & 3.5 & 5.5 & 5.0 & 8.25 & 10.0 & 4.0 & 9.28 & 22.18 \\

\bottomrule
\end{tabular}
\end{table}


==> tables/screenspot.tex <==
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c}{\textbf{Mobile}} & \multicolumn{2}{c}{\textbf{Desktop}} & \multicolumn{2}{c}{\textbf{Web}} & \textbf{Desktop} & \textbf{Avg.} \\ 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
& & \multicolumn{1}{c}{\textbf{Text}} & \multicolumn{1}{c}{\textbf{Icon/Widget}} & \multicolumn{1}{c}{\textbf{Text}} & \multicolumn{1}{c}{\textbf{Icon/Widget}} & \multicolumn{1}{c}{\textbf{Text}} & \multicolumn{1}{c}{\textbf{Icon/Widget}} & \textbf{Avg.} & \\ 
\midrule
GPT-4 & SeeClick & 76.6 & 55.5 & 68.0 & 28.6 & 40.9 & 23.3 & 48.3 & 48.8 \\ 
GPT-4 & OmniParser & 93.9 & 57.0 & 91.3 & 63.6 & 81.3 & 51.0 & 77.5 & 73.0 \\ 
GPT-4 & UGround & 90.1 & 70.3 & 87.1 & 55.7 & 85.7 & 64.6 & 71.4 & 75.6 \\ 
GPT-4o & SeeClick & 81.0 & 59.8 & 69.6 & 33.6 & 43.9 & 26.2 & 51.6 & 52.3 \\ 
GPT-4o & UGround & 93.4 & 76.9 & 92.8 & 67.9 & 88.7 & 68.9 & 80.4 & 81.4 \\ 
\midrule
\multicolumn{2}{c}{GPT-4} & 22.6 & 24.5 & 20.2 & 11.8 & 9.2 & 8.8 & 16.0 & 16.2 \\ 
\multicolumn{2}{c}{GPT-4o} & 20.2 & 24.9 & 21.1 & 23.6 & 12.2 & 7.8 & 22.4 & 18.3 \\ 
\multicolumn{2}{c}{CogAgent} & 67.0 & 24.0 & 74.2 & 20.0 & 70.4 & 28.6 & 47.1 & 47.4 \\ 
\multicolumn{2}{c}{SeeClick} & 78.0 & 52.0 & 72.2 & 30.0 & 55.7 & 32.5 & 51.1 & 53.4 \\ 
\multicolumn{2}{c}{Qwen2-VL} & 75.5 & 60.7 & 76.3 & 54.3 & 35.2 & 25.7 & 65.3 & 55.3 \\ 
\multicolumn{2}{c}{UGround} & 82.8 & 60.3 & 82.5 & 63.6 & 80.4 & 70.4 & 73.1 & 73.3 \\ 
\multicolumn{2}{c}{AGUVIS-7B} & 95.6 & 77.7 & 93.8 & 67.1 & 88.3 & 75.2 & 80.5 & 84.4 \\ 
\multicolumn{2}{c}{AGUVIS-72B} & 94.5 & 85.2 & 95.4 & 77.9 & 91.3 & 85.9 & 86.7 & 89.2 \\ 
\midrule[\heavyrulewidth]
\multicolumn{2}{c}{\textbf{AgentNet-7B}} & 81.3 & 51.5 & 88.3 & 76.7 & 92.3 & 70.0 & 82.5 & 76.9 \\
\multicolumn{2}{c}{\textbf{AgentNet-A3B}} & & & & & & & & 91.4\\
\multicolumn{2}{c}{\textbf{AgentNet-7B w/ Aguvis}} & 94.5 & 78.6 & 94.9 & 77.1 & 90.4 & 79.1 & 86.0 & 86.7 \\
% \multicolumn{2}{c}{\textbf{AgentNet-72B w/ Aguvis}} & & & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison of different models on Screenspot.}
\label{tab:screenspot}
\end{table}

==> tables/screenspot_pro.tex <==
\begin{table}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l ccc ccc ccc ccc ccc ccc ccc}
\toprule
\multirow{2}{*}{Agent Model} & \multicolumn{3}{c}{\textbf{Development}} & \multicolumn{3}{c}{\textbf{Creative}} & \multicolumn{3}{c}{\textbf{CAD}} & \multicolumn{3}{c}{\textbf{Scientific}} & \multicolumn{3}{c}{\textbf{Office}} & \multicolumn{3}{c}{\textbf{OS}} & \multicolumn{3}{c}{\textbf{Avg}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
& \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} & \textbf{Text} & \textbf{Icon} & \textbf{Avg} \\
\midrule
QwenVL-7B (Bai et al., 2023b) & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.7 & 0.0 & 0.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.1 & 0.0 & 0.1 \\
GPT-4v (Hurst et al., 2024) & 1.3 & 0.0 & 0.7 & 1.0 & 0.0 & 0.6 & 2.0 & 0.0 & 1.5 & 2.1 & 0.0 & 1.2 & 1.1 & 0.0 & 0.9 & 0.0 & 0.0 & 0.0 & 1.3 & 0.0 & 0.8 \\
SeeClick (Cheng et al., 2024) & 0.6 & 0.0 & 0.3 & 1.0 & 0.0 & 0.6 & 2.5 & 0.0 & 1.9 & 3.5 & 0.0 & 2.0 & 1.1 & 0.0 & 0.9 & 2.8 & 0.0 & 1.5 & 1.8 & 0.0 & 1.1 \\
Qwen2-VL-7B (Wang et al., 2024c) & 2.6 & 0.0 & 1.3 & 1.5 & 0.0 & 0.9 & 0.5 & 0.0 & 0.4 & 6.3 & 0.0 & 3.5 & 3.4 & 1.9 & 3.0 & 0.9 & 0.0 & 0.5 & 2.5 & 0.2 & 1.6 \\
OS-Atlas-4B (Wu et al., 2024b) & 7.1 & 0.0 & 3.7 & 3.0 & 1.4 & 2.3 & 2.0 & 0.0 & 1.5 & 9.0 & 5.5 & 7.5 & 5.1 & 3.8 & 4.8 & 5.6 & 0.0 & 3.1 & 5.0 & 1.7 & 3.7 \\
ShowUT-2B (Lin et al., 2024b) & 16.9 & 1.4 & 9.4 & 9.1 & 0.0 & 5.3 & 2.5 & 0.0 & 1.9 & 13.2 & 7.3 & 10.6 & 15.3 & 7.5 & 13.5 & 10.3 & 2.2 & 6.6 & 10.8 & 2.6 & 7.7 \\
CogAgent-18B (Hong et al., 2024) & 14.9 & 0.7 & 8.0 & 9.6 & 0.0 & 5.6 & 7.1 & 3.1 & 6.1 & 22.2 & 1.8 & 13.4 & 13.0 & 0.0 & 10.0 & 5.6 & 0.0 & 3.1 & 12.0 & 0.8 & 7.7 \\
Aria-U1 (Yang et al., 2024a) & 16.2 & 0.0 & 8.4 & 23.7 & 2.1 & 14.7 & 7.6 & 1.6 & 6.1 & 27.1 & 6.4 & 18.1 & 20.3 & 1.9 & 16.1 & 4.7 & 0.0 & 2.6 & 17.1 & 2.0 & 11.3 \\
UGround-7B (Gou et al., 2024a) & 26.6 & 2.1 & 14.7 & 27.3 & 2.8 & 17.0 & 14.2 & 1.6 & 9.7 & 31.9 & 2.7 & 19.3 & 31.6 & 11.3 & 27.0 & 17.8 & 0.0 & 9.7 & 25.0 & 2.8 & 16.5 \\
Claude Computer Use (Anthropic, 2024b) & 22.0 & 3.9 & 12.6 & 25.9 & 3.4 & 16.8 & 14.5 & 3.7 & 11.9 & 33.9 & 15.8 & 25.8 & 30.1 & 16.3 & 26.9 & 11.0 & 4.5 & 8.1 & 23.4 & 7.1 & 17.1 \\
OS-Atlas-7B (Wu et al., 2024b) & 33.1 & 1.4 & 17.7 & 28.8 & 2.8 & 17.9 & 12.2 & 4.7 & 10.3 & 37.5 & 7.3 & 24.4 & 33.9 & 5.7 & 27.4 & 27.1 & 4.5 & 16.8 & 28.1 & 4.0 & 18.9 \\
UGround-V1-7B (Gou et al., 2024a) & - & - & 35.5 & - & - & 27.8 & - & - & 13.5 & - & - & 38.8 & - & - & 48.8 & - & - & 26.1 & - & - & 31.1 \\
UI-TARS-2B & 47.4 & 4.1 & 26.4 & 42.9 & 6.3 & 27.6 & 17.8 & 4.7 & 14.6 & 56.9 & 17.3 & 39.8 & 50.3 & 17.0 & 42.6 & 21.5 & 5.6 & 14.3 & 39.6 & 8.4 & 27.7 \\
UI-TARS-7B & 58.4 & 12.4 & 36.1 & 50.0 & 9.1 & 32.8 & 20.8 & 9.4 & 18.0 & 63.9 & 31.8 & 50.0 & 63.3 & 20.8 & 53.5 & 30.8 & 16.9 & 24.5 & 47.8 & 16.2 & 35.7 \\
UI-TARS-72B & 63.0 & 17.3 & 40.8 & 57.1 & 15.4 & 39.6 & 18.8 & 12.5 & 17.2 & 64.6 & 20.9 & 45.7 & 63.3 & 26.4 & 54.8 & 42.1 & 15.7 & 30.1 & 50.9 & 17.5 & 38.1 \\
\midrule[\heavyrulewidth]
\textbf{AgentNet-7B} &  &  &  &  &  &  &  & & & & & & & & & & & & & & 21.5 \\
\textbf{AgentNet-A3B} & & & & & & & & & & & & & & & & & & & & & 28.5\\
\textbf{AgentNet-7B w/ Aguvis} &  &  &  &  &  &  &  & & & & & & & & & & & & & & 23.3\\
% \textbf{AgentNet-72B w/ Aguvis} & & & & & & & & & & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Comparison of various models on ScreenSpot-Pro.}
\label{tab:screenspot_pro}
\end{table}
